Robbing the Fed: Directly Obtaining Private Data in Federated Learning with Modified Models

Federated learning has quickly gained popularity with its promises of increased user privacy and efficiency. Previous works have shown that federated gradient updates contain information that can be used to approximately recover user data in some situations. These previous attacks on user privacy have been limited in scope and do not scale to gradient updates aggregated over even a handful of data points, leaving some to conclude that data privacy is still intact for realistic training regimes. In this work, we introduce a new threat model based on minimal but malicious modifications of the shared model architecture which enable the server to directly obtain a verbatim copy of user data from gradient updates without solving difficult inverse problems. Even user data aggregated over large batches -- where previous methods fail to extract meaningful content -- can be reconstructed by these minimally modified models.

==> notes.tex <==
\section*{Temporary notes}
\begin{itemize}
    \item If we can get some numbers for failures in large batches (with the 3-bin trick) that'd be super impactful
    \item I think this also works for FedAVG (FL with multiple local update steps) industry people probs like that
    
    \item Threat models: A) arbitrary code execution -> this is of course dumb, but even here and attack could be found easily by looking at network bandwidth audits. Attacks that send user data instead of the gradient need to handle batches. Against these attacks, a simple defense on the user side would be that data is sandboxed and processed separately and averaged on the user-side, and that only the final average is sent. If the attacker writes the image into the gradient, then averaging still destroys it. [Only our technique will later circumvent this]. Aside from the fact, that all of these attacks are easily visible in code audits. Our attack, however, uses the federated learning system that might be hardcoded into a system, entirely normally - just with a minimal architectural change.
    
    \item Point out in the beginning that it is trivially true that larger models (as in parameter size) have a larger gradient and thus leak more info, but we that we will show that not all models are created equal in this way.

    
    \item The linear model + cross-entropy example is optimal. For a batch that contains each of the labels only once, exactly 100\% of the gradient signal can be directly converted into input data. We can use this as a nice motivation (and compare to the ResNet-50 from see through gradients) which has a conversion ratio of much less (in terms of gradient parameters to recovered images). We can then note that this is a very specific construction that hinges on 1) unique labels and 2) the sparsity of cross-entropy loss, making it inapplicable in practice, but ... we can then segway into imprint modules which do this much better, without label info, for any possible data type and everywhere in the network with arbitrary many bins
    \item We show that with only N\% more parameters, we can leak 100*N\% more data or something like that 
    \item Cool plots:
    \begin{itemize}
        \item IIP score for a batch of 8(?) images for a Resnet of varying widths for an optimization-based attack (score will increase slowly as parameters increase) vs
        \item IIP-score for a batch of (?) many images for our module with increasing number of bins (IIP score will increase quickly as parameters=bins increase)
        \item Score vs batch size for a fixed number of bins
    \end{itemize}
    
    Images to show:
    \begin{itemize}
        \item Linear stuff?
        \item imprint module in the beginning
        \item imprint module somewhere in a network(is this cool?)
    \end{itemize}
    
    \item I've seen (ethics) reviewers at previous neurips/iclr requiring something about defenses. We can actually propose a defense against this. The defense would measure gradient sparsity on the user side (in the sense of counting how many entries in the averaged gradient are actually only coming from a single data point. This is of course super expensive and not a great practical defense (requiring tons of per-example gradients), but cool from a method standpoint and something to assuage questions about defenses.
    [UPDATE:] Our new ReLU activation imprint is even better, because it does not expose a simple sparsity pattern in the data. We could even do our attack, but with a secret order of bins, which is only known to the server. Half of the layer could also just do normal things instead of binning, making it even harder to analyze the attack.
    \item paper take-away: Small changes can have a disproportionate effect and breach FL, even on large batches. Designers of FL systems (and user of e.g. open-sourced FL projects) need to be aware of these vulnerabilities. At the same time, this is difficult as stakeholders (e.g. hospitals) might not have the know-how to gauge if a given architecture is especially vulnerable. Vetted architectures?
    \item good regularizers help reconstruction on images, but not on tabular. This always works everywhere
    \item given that we already assume that the server intends to do data theft, it is a small leap to think that this actor might also do small model modifications!
    
    \item Secure aggregation is pointless with sparse data (and effectively equivalent to secure shuffling, which hides from which user data came). Our approach artificially generates sparse locations in the gradient of any model by a clever choice of parameters.[UPDATE: THIS IS NOT TRUE ANYMORE FOR THE NEW APPROACH]
    
    \item This attack can also be used to verify a user has a particular piece of data: Simply compute precise average value for this data points (e.g. its brightness), and set bins closely around this value. If the data returns from the user update in this way, then it truly does belong to this user.
    
    \item maybe we should sell the hardtanh part as an attack against multiple local update steps?
    \item We can easily just shuffle the bins to make it a bit less obvious
\end{itemize}

Stuff to point out somewhere:
\begin{itemize}
    \item We show cool images because previous work has shown cool images (and ours are even cooler), but we stress that the attack is entirely data-agnostic and can also work for tabular data, text etc...
    \item The imprint module can even lie dormant as an attention/FC layer undetected by the proposed defense - it is only when the right combination of parameters is sent from the server, that the attack activates.
\end{itemize}
